Boosting Earth System Model Outputs And Saving PetaBytes in their Storage Using Exascale Climate Emulators

We present the design and scalable implementation of an exascale climate emulator for addressing the escalating computational and storage requirements of high-resolution Earth System Model simulations. We utilize the spherical harmonic transform to stochastically model spatio-temporal variations in climate data. This provides tunable spatio-temporal resolution and significantly improves the fidelity and granularity of climate emulation, achieving an ultra-high spatial resolution of 0.034 (approximately 3.5 km) in space. Our emulator, trained on 318 billion hourly temperature data points from a 35-year and 31 billion daily data points from an 83-year global simulation ensemble, generates statistically consistent climate emulations. We extend linear solver software to mixed-precision arithmetic GPUs, applying different precisions within a single solver to adapt to different correlation strengths. The PaRSEC runtime system supports efficient parallel matrix operations by optimizing the dynamic balance between computation, communication, and memory requirements. Our BLAS3-rich code is optimized for systems equipped with four different families and generations of GPUs, scaling well to achieve 0.976 EFlop/s on 9,025 nodes (36,100 AMD MI250X multichip module (MCM) GPUs) of Frontier (nearly full system), 0.739 EFlop/s on 1,936 nodes (7,744 Grace-Hopper Superchips (GH200)) of Alps, 0.243 EFlop/s on 1,024 nodes (4,096 A100 GPUs) of Leonardo, and 0.375 EFlop/s on 3,072 nodes (18,432 V100 GPUs) of Summit.

==> ET.tex <==

 
Evapotranspiration (ET) includes water evaporation and transpiration processes to move the water from the earth's surface into the atmosphere. The evaporation process happens when the soil is water-saturated and starts to runoff water to the surface. With the sun heating,  the water is evaporated and goes into the air. The transpiration process involves the loss of water vapor through the stomata of plants and the effect of hot weather~\cite{cascone2019evapotranspiration}. Evapotranspiration plays an essential part in the earth's hydrologic cycle. Measuring it can help in watershed management and agricultural irrigation. It is also a critical factor in many fields such as climatology, agronomy, meteorology, ecology, and environmental science~\cite{liu2019simulation, petkovic2020neuro,talebizadeh2018simultaneous}.






==> attributes.tex <==
%!TEX root = manuscript_gb.tex
\ifthenelse {\boolean{GuideOn}} {
{\bf 
(use a table listing each attribute title and value in a separate row)

Category of achievement (1+ of:  scalability, time-to-solution, peak performance)

Type of method used (1 of:  explicit, implicit, both explicit and implicit, semi-implicit, n/a)

Results reported on the basis of (1 of:  whole application including I/O; whole application except I/O; kernel only; other [specify])

Precision reported (1 of:  single precision, double precision, mixed precision)

System scale (1 of:  results measured on full-scale system, projected from results of smaller system, other [specify])

Measurement mechanism (1 of:  timers, FLOP count, static analysis tool, performance modeling, other [specify])
}
} {
}
% $1{,}038{,}240$ spatial locations across the globe\\
%              & at a spatial resolution of $0.25^\circ$
\begin{center}
\begin{table}[h]
\begin{tabular}{l|l}
\hline
%Performance Attributes       & Our submission                                               \\ \hline
Problem size                 &  \spatiallocations spatial locations across the\\
              & globe at a spatial resolution of \resolutionDegree \\&($\sim$\resolutionKm) \\
\hline
Category of achievement      & Scalability
                            and peak performance\\ Type of method used          & Spherical Harmonic Transform (SHT) \\
& and Cholesky factorization                \\ 
\hline
Results reported on basis of & Cholesky factorization                   \\ 
Precision reported           & Double and mixed-precision
              \\ 
System scale                 & - \frontierPerf EFlop/s on \frontierNode nodes of \\
                             &  Frontier (\frontierGPU AMD MI250X \\&multi-chip module (MCM) GPUs)   \\& equivalent to \frontierDIE AMD Graphics  \\& Compute Dies (GCDs) \\
 %& - projected to $\sim 1.04$ EFlops/s on $8{,}192$ nodes\\
                & - \ALPSPerf EFlop/s on \ALPSNode nodes of \\
                &Alps (\ALPSGPU NVIDIA Grace-Hopper \\&Superchips (GH200))\\
                & - \leonardoPerf EFlop/s on \leonardoNode nodes of \\
                &Leonardo (\leonardoGPU NVIDIA A100 GPUs)\\
                & - \summitPerf EFlop/s on \summitNode nodes of \\
                & Summit (\summitGPU NVIDIA V100 GPUs) \\
\hline
Measurement mechanism        & Timers, Flops  \\ 
\hline
\end{tabular}
\end{table}
\end{center}
%\footnotetext[1]{To be extended to full-scale of Frontier.}

%\todo{Problem Size should be 33189120}
%\todo{Frontier GPU should be 16384}

==> justification.tex <==
%!TEX root = manuscript_gb.tex
\ifthenelse{\boolean{GuideOn}}{
\textbf{(50 word max)}}

%Synergistic combination of mixed-precision computation
%and 
%dynamic task-based runtime system for on-demand data conversion and data movement reduction. Scalability on 5,000 Frontier nodes (30,000 GPUs)
%for Spherical Harmonic Transform (SHT).
%Performance speedup up to 8X over FP64
%execution achieving 0.5 Eflops/s, while attaining application-worthy accuracy.
%Incorporation into path-finding software framework
%for geostatistical applications.
{\color {red}
Exascale climate emulator developed using 318 billion hourly and 31 billion daily observations for generating climate emulations at ultra-high spatial resolution~(\resolution). Modeling climate data using spherical harmonics. Mixed-precision computations. \parsec dynamic runtime system. 
Running on \frontierNode nodes on Frontier, \ALPSNode nodes on Alps, \leonardoNode nodes on Leonardo, and \summitNode nodes on Summit, with the hybrid Flop/s rates \frontierPerf EFlop/s, \ALPSPerf EFlop/s, \leonardoPerf EFlop/s, and \summitPerf EFlop/s, respectively.}
%\newpage

%the performance in different precision modes are as follows: FP16 computation achieves {\color{red}??? PFLOPS (???\% of the FP-64 theoretical peak)}, FP32 computation reaches {\color{red}??? PFLOPS (???\% of the FP-64 theoretical peak)}, and FP64 computation attains {\color{red}??? PFLOPS (???\% of the FP-64 theoretical peak)}. Additionally, the combined FP64/FP32/FP16 performance is {\color{red}??? PFLOPS (???\% of the FP-64 theoretical peak)}.





% \todo{Updated the whole paper: 16K to 48K; 9M to 10M}
